Toward Scene Graph and Layout Guided Complex 3D Scene Generation

Recent advancements in object-centric text-to-3D generation have shown impressive results. However, generating complex 3D scenes remains an open challenge due to the intricate relations between objects. Moreover, existing methods are largely based on score distillation sampling (SDS), which constrains the ability to manipulate multiobjects with specific interactions. Addressing these critical yet underexplored issues, we present a novel framework of Scene Graph and Layout Guided 3D Scene Generation (GraLa3D). Given a text prompt describing a complex 3D scene, GraLa3D utilizes LLM to model the scene using a scene graph representation with layout bounding box information. GraLa3D uniquely constructs the scene graph with single-object nodes and composite super-nodes. In addition to constraining 3D generation within the desirable layout, a major contribution lies in the modeling of interactions between objects in a super-node, while alleviating appearance leakage across objects within such nodes. Our experiments confirm that GraLa3D overcomes the above limitations and generates complex 3D scenes closely aligned with text prompts.

==> pseudo_code/alg.tex <==
% \begin{algorithm}
% 	\caption{Target View Depth Estimation}
%  \label{alg:1}
% 	\begin{algorithmic}[1]
%         \State Initialize points as an empty array
%         \For {each k in 1, 2, ..., K}
%             \State Create grid by meshing height (H) and width (W)
%             \State Project the grid onto the coordinate $\xi_k$
%             \State Scale the grid by factor $D_k$
%             \State Transform the grid to the world coordinate based on $\xi_k$
%             \State Add the transformed grid to the points array
%         \EndFor
%         \State Convert points to target view using $\xi_k$ coordinate
%         \State Reproject the points to the $\xi_k$ image plane
%         \State Define target depth as the second element of points
%         \State Convert the points' coordinates to integers
%         \State Compute the difference between the original and integer coordinates
%         \State Apply weights to target depth and normalize using the computed difference
%         \State Return the processed target depth
% 	\end{algorithmic} 
% \end{algorithm} 

\begin{algorithm}[tb]
\caption{Estimation of Depth in Target View}
\label{alg:algorithm}
\textbf{Input}: Depth predictions of each source view $D_{1:K}$, camera pose of each source view $\xi_{1:K}$, target camera pose $\xi_T$\\
\textbf{Data}: Image size: (H, W), camera pose of the world coordinate $\xi_w$
\begin{flushleft}
\textbf{Output}: Target view depth estimation $D_T$
\end{flushleft}
\begin{algorithmic}[1] %[1] enables line numbers
% \STATE Create an empty array $A$ as points
\STATE $A$ $\leftarrow$ empty array()
\FOR{$k$ = $1,...,K$}
    % \STATE Generate grid $g$ by meshing the dimensions of height (H) and width (W)
    \STATE $g$ $\leftarrow$ meshgrid(H, W)
    \STATE Project $g$ into the coordinate system defined by $\xi_k$
    \STATE Multiply $g$ by the corresponding depth prediction $D_k$
    % \STATE Transform $g$ to world coordinates using $\xi_k$
    \STATE $g$ $\leftarrow$ \textbf{Transform}($g$, $\xi_k$, $\xi_{w}$)
    \STATE Append $g$ to the array $A$
\ENDFOR
% \STATE Transform points $A$ into target view coordinates $\xi_T$
\STATE $A$ $\leftarrow$ \textbf{Transform}($A$, $\xi_{w}$, $\xi_T$)
\STATE Reproject $A$ onto the $\xi_T$ image plane
% \STATE Extract the third component (Z-axis) of points $A$ and set it to $Z$
\STATE $Z$ $\leftarrow$ the third element (Z-axis) of points $A$ 
% \STATE Preserve points $A$ in variable $\textit{tmp}$
% \STATE $\textit{tmp}$ $\leftarrow$ $A$  \textcolor{red}{seems do not need explicitly say this?}
\STATE $A'$ $\leftarrow$ round the first two elements of $A$ to integer values
% \STATE Calculate the difference of first two elements between $\textit{tmp}$ and $A$, set it to weight $W$
% \STATE $W$ $\leftarrow$ the difference of first two elements between $\textit{tmp}$ and $A$
\STATE $W$ $\leftarrow$ The first two elements of ($A'$ - $A$)
\STATE Weight and normalize $Z$ using weight $W$
\STATE Set the depth of target view $D_T$ to $Z$ based on the index of the first two elements of $A'$
\RETURN Estimated depth of target view $D_T$
\STATE
\STATE \textit{/* Function */}
\STATE \textbf{Transform}(point, $\xi_1$, $\xi_2$):
\RETURN transform point from coordinate $\xi_1$ to $\xi_2$
\end{algorithmic}
% \vspace{-2mm}
\end{algorithm}

